Assessing Spectroscopic-Binary Multiplicity Properties Using Robo-AO Imaging

We present higher-order multiplicity results for 60 solar-type spectroscopic binaries based on 0.75 micron imaging data taken by the Robotic Adaptive Optics system (Robo-AO) at the Kitt Peak 2.1m telescope. Our contrast curves show sensitivity of up to ~5 mag at ~1 arcsecond separation. We find tertiary companions for 62% of our binaries overall, but find this fraction is a strong function of the inner binary orbital period; it ranges from ~47% for P_{binary} > 30 days to as high as ~90% for P_{binary} <= 5 days. We similarly find increasing tertiary companion frequency for shorter period binaries in a secondary sample of Kepler eclipsing binaries observed by Robo-AO. Using Gaia distances, we estimate an upper limit orbital period for each tertiary companion and compare the tertiary-to-binary period ratios for systems in the field versus those in star-forming regions. Taken all together, these results provide further evidence for angular momentum transfer from three-body interactions, resulting in tight binaries with tertiaries that widen from pre-main-sequence to field ages.

==> Extras/packages.tex <==
% This is the set of packages to use across the document

\usepackage[export]{adjustbox}
\usepackage{subcaption}
\usepackage{graphics}
\usepackage{hyperref}

%\usepackage{longtable} % for 'longtable' environment



\hypersetup{
    pdfauthor=Stefan Laos,
    pdftitle=Work in Progress,
    colorlinks=true,
    citecolor=blue,
    linkcolor=black,
    urlcolor=cyan}

